An Approach to Detecting Bugs in Pattern-Based Bug Detectors

Static bug finders have been widely-adopted by developers to find bugs in real world software projects. They leverage predefined heuristic static analysis rules to scan source code or binary code of a software project, and report violations to these rules as warnings to be verified. However, the advantages of static bug finders are overshadowed by such issues as uncovered obvious bugs, false positives, etc. To improve these tools, many techniques have been proposed to filter out false positives reported or design new static analysis rules. Nevertheless, the under-performance of bug finders can also be caused by the incorrectness of current rules contained in the static bug finders, which is not explored yet. In this work, we propose a differential testing approach to detect bugs in the rules of four widely-used static bug finders, i.e., SonarQube, PMD, SpotBugs, and ErrorProne, and conduct a qualitative study about the bugs found. To retrieve paired rules across static bug finders for differential testing, we design a heuristic-based rule mapping method which combines the similarity in rules description and the overlap in warning information reported by the tools. The experiment on 2,728 open source projects reveals 46 bugs in the static bug finders, among which 24 are fixed or confirmed and the left are awaiting confirmation. We also summarize 13 bug patterns in the static analysis rules based on their context and root causes, which can serve as the checklist for designing and implementing other rules and or in other tools. This study indicates that the commonly-used static bug finders are not as reliable as they might have been envisaged. It not only demonstrates the effectiveness of our approach, but also highlights the need to continue improving the reliability of the static bug finders.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> tab/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> tab/bug_false_positive_old.tex <==
\begin{table*}[ht!]
\caption{False positive bugs in the examined static bug finders}
\centering
\footnotesize
\begin{tabular}{p{3cm}|p{7.5cm}|p{6cm}}
\hline
\textbf{Bug pattern} & \textbf{Example} & \textbf{Involved rules (occurrence times)} \\ 
\hline
\multirow{3}{*}{\shortstack[l]{\textbf{\textit{P11.} Poor handling of } \\\textbf{method with same name}}} & \multirow{3}{*}{\shortstack[l]{ \textit{UseNotifyAllInsteadOfNotify} should warn \textit{Object.notify()}, but \\wrongly warns \textit{notify(para)} method in other class, \\e.g., getEventThread().notify(input);}} & \textit{PMD}: SuspiciousEqualsMethodName (24)\\
 &  & \textit{PMD}: UseNotifyAllInsteadOfNotify (12) \\
& & \textit{SonarQube}: Object.finalize() should remain protected (versus public) when overriding (6)   \\
 \hline
\multirow{3}{*}{\shortstack[l]{\textbf{\textit{P12.} Setting over-sized}\\ \textbf{scope}}} & \multirow{3}{*}{\shortstack[l]{\textit{AvoidThrowingNullPointerException} wrongly warns the \\ expression with \textit{NullPointerException} yet without \textit{Throwing}, \\ e.g., Exception e = new NullPointerException(``msg'');}} & 
\textit{PMD}: AvoidThrowingNullPointerException (18) \\
 &  & \textit{SpotBugs}: SF\_SWITCH\_NO\_DEFAULT (11)  \\
& & \textit{PMD}: AvoidCallingFinalize (6)\\
 \hline
\multirow{2}{*}{\shortstack[l]{\textbf{\textit{P13.} Neglecting corner}\\ \textbf{case}}} & \multirow{2}{*}{\shortstack[l]{\textit{MissingBreakInSwitch} wrongly warns the \textit{switch} expression \\ without \textit{break} in the last \textit{case} statement;}} & 
\textit{PMD}: MissingBreakInSwitch (841) \\
 &  & \textit{PMD}: AvoidReassigningLoopVariables (188) \\
\hline
\end{tabular}
\label{tab:bug_false_positive}
\end{table*}

==> tab/bug_rule_definition_old.tex <==
\begin{table*}[ht!]
\caption{False negative bugs (about rule definition) in the examined static bug finders.}
\centering
\footnotesize
\begin{tabular}{p{3cm}|p{7.5cm}|p{6cm}}
\hline
\textbf{Bug Patterns} & \textbf{Example} & \textbf{Involved rules (occurrence times)} / \textcolor{blue}{C} indicates fixed/confirmed bug\\ 
\hline
\multirow{4}{*}{\shortstack[l]{\textbf{\textit{P8.} Miss comparable}\\ \textbf{method}}} & \multirow{4}{*}{\shortstack[l]{\textit{UseLocaleWithCaseConversions} fails with \textit{String.format()}, \\ while works with \textit{String.toLowerCase()/toUpperCase();}}} & \textit{PMD}: UseLocaleWithCaseConversions (464)  \\
 &  & \textit{ErrorProne}: BoxedPrimitiveEquality (14)  \\
 & & \textit{SonarQube}: Java.lang.Error should not be extended (7)  / \textcolor{blue}C \\
  &  & \textit{SonarQube}: Execution of the Garbage Collector should be triggered only by the JVM (7)  \\
 \hline
 \multirow{3}{*}{\shortstack[l]{\textbf{\textit{P9.} Miss comparable}\\ \textbf{data type or operation}}} & \multirow{3}{*}{\shortstack[l]{\textit{ICAST\_INTEGER\_MULTIPLY\_CAST\_TO\_LONG} fails with \\ \textit{shift} operation, while works with \textit{multiply} operation; }} & \textit{SonarQube}: Redundant modifiers should not be used (1271) \\
%  &  & \textit{SonarQube}: Non-primitive fields should not be volatile (538)   \\
& & \textit{PMD}: AvoidArrayLoops (362) \\
 &  & \textit{SpotBugs}: ICAST\_INTEGER\_MULTIPLY\_CAST\_ TO\_LONG (39) \\
 \hline
\multirow{2}{*}{\shortstack[l]{\textbf{\textit{P10.} Miss subclass}\\ \textbf{or superclass}}} & \multirow{2}{*}{\shortstack[l]{\textit{AvoidCatchingThrowable} fails in the subclass of \textit{Throwable},\\  e.g., catch (Error e);}} & \textit{PMD}: ReturnEmptyArrayRatherThanNull (677) \\
 &  & \textit{PMD}: AvoidCatchingThrowable (41)   \\
%  \hline
%  \multirow{3}{*}{Others}  &  \multirow{3}{*}{N/A. Delete this category might be better} & \textit{PMD}: SimplifyBooleanExpressions (623) \\
%   & &  \textit{PMD}: NonStaticInitializer (568) \\
%   & & \textit{PMD}: SimplifyBooleanReturns (181)\\
\hline
\end{tabular}
\label{tab:bug_rule_define}
\end{table*}

==> tab/bug_rule_implement-auto.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\large
\begin{tabular}{|l|l|l|}
\hline
\textbf{Bug pattern}                                                                                                & \textbf{Example}                                                                                                                                                                                                                                                                    & \textbf{Involved static analysis rules (occurrence times)}                                                                       \\ \hline
\multirow{5}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Fail in \\ special data type\end{tabular}}}}             & \multirow{5}{*}{\textit{\begin{tabular}[c]{@{}l@{}}Object should not be created only to getClass \\ fails with Array, while works with ArrayList;\end{tabular}}}                                                                                                                    & \textit{PMD: SingularField (327)}                                                                                                \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{\begin{tabular}[c]{@{}l@{}}SonarQube: String function use should be optimized \\ for single characters (8)\end{tabular}} \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{\begin{tabular}[c]{@{}l@{}}SonarQube: Objects should not be created only to \\ getClass (5)\end{tabular}}                \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{PMD: RedundantFieldInitializer (3)}                                                                                      \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & SpotBugs: ICAST\_BAD\_SHIFT\_AMOUNT (3)                                                                                          \\ \hline
\multirow{5}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Fail in \\ compound expression\end{tabular}}}}           & \multirow{5}{*}{\textit{\begin{tabular}[c]{@{}l@{}}QBA QUESTIONABLE BOOLEAN ASSIGNMENT fails\\ when compound expression is involved, e.g.,\\ if (scanning = b == false);\end{tabular}}}                                                                                             & \textit{ErrorProne: ToStringReturnsNull (28)}                                                                                    \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{SpotBugs: QBA QUESTIONABLE BOOLEAN ASSIGNMENT (26)}                                                                      \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{SpotBugs: SA LOCAL SELF ASSIGNMENT (26)}                                                                                 \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{SonarQube: Variables should not be self-assigned (5)}                                                                    \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{\begin{tabular}[c]{@{}l@{}}SonarQube: Fields should not be initialized to \\ default values (3)\end{tabular}}            \\ \hline
\multirow{4}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Fail in \\ implicit operation\end{tabular}}}}            & \multirow{4}{*}{\textit{\begin{tabular}[c]{@{}l@{}}IntLongMath (Expression of type int may \\ overflow before assigning to a long) fails \\ when used in comparison expression \\ (i.e., implicit assign), \\ e.g., if (score \textgreater{}= level * level * 1000);\end{tabular}}} & \textit{ErrorProne: IntLongMath (135)}                                                                                           \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{\begin{tabular}[c]{@{}l@{}}SonarQube: Static fields should not be updated in \\ constructors (72)\end{tabular}}          \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{SpotBugs: DMI INVOKING TOSTRING ON ARRAY (53)}                                                                           \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{ErrorProne: ArrayEquals (11)}                                                                                            \\ \hline
\multirow{4}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Fail in \\ multiple calling\\ operations\end{tabular}}}} & \multirow{4}{*}{\textit{\begin{tabular}[c]{@{}l@{}}AvoidPrintStackTrace fails when involving \\ multiple calling operations, e.g., \\ json.excpetion().printStackTrace();\end{tabular}}}                                                                                            & \textit{PMD: UseCollectionIsEmpty (399)}                                                                                         \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{PMD: AvoidPrintStackTrace (20)}                                                                                          \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{PMD: ClassCastExceptionWithToArray (5)}                                                                                  \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{PMD: DontCallThreadRun (5)}                                                                                              \\ \hline
\multirow{3}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Fail in \\ separated expressions\end{tabular}}}}         & \multirow{3}{*}{\textit{\begin{tabular}[c]{@{}l@{}}UseProperClassLoader fails when getClassLoader \\ is used in separated expressions, \\ e.g., Foo foo = new Foo();ClassLoader \\ classLoader = foo.getClassLoader();\end{tabular}}}                                               & \textit{PMD: UseProperClassLoader (68)}                                                                                          \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{ErrorProne: ToStringReturnsNull (28)}                                                                                    \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{PMD: InstantiationToGetClass (19)}                                                                                       \\ \hline
\multirow{3}{*}{\textit{\textbf{\begin{tabular}[c]{@{}l@{}}Fail in \\ unnecessary brackets\end{tabular}}}}          & \multirow{3}{*}{\textit{\begin{tabular}[c]{@{}l@{}}SimplifyConditional fails with if(rhs != null \\ \&\& (rhs instanceof CodeLocation)), yet works \\ when deleting the unnecessary brackets on \\ the second condition;\end{tabular}}}                                             & \textit{PMD: ReturnEmptyArrayRatherThanNull (770)}                                                                               \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{PMD: SimplifyConditional (109)}                                                                                          \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{\begin{tabular}[c]{@{}l@{}}SonarQube: Switch statements should not contain \\ non-case labels (39)\end{tabular}}         \\ \hline
\multirow{3}{*}{\textit{\textbf{Fail in variables}}}                                                                & \multirow{3}{*}{\textit{\begin{tabular}[c]{@{}l@{}}FinalFieldCouldBeStatic fails when assigning \\ to an expression, yet works when assigning to\\ a constant, e.g.,\\ private final double HALF PI = Math.PI  0.5;\end{tabular}}}                                                 & \textit{PMD: FinalFieldCouldBeStatic (209)}                                                                                      \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     & \textit{PMD: AvoidDecimalLiteralsInBigDecimalConstructor (20)}                                                                   \\ \cline{3-3} 
                                                                                                                    &                                                                                                                                                                                                                                                                                     &                                                                                                                                  \\ \hline
\end{tabular}%
}
\end{table*}

==> tab/bug_rule_implement_old.tex <==
\begin{table*}[ht!]
\caption{False negative bugs (about rule implementation) in the examined static bug finders}
\centering
\footnotesize
\begin{tabular}{p{2.8cm}|p{7.5cm}|p{6cm}}
\hline
\textbf{Bug pattern} & \textbf{Example} & \textbf{Involved rules (occurrence times)} / \textcolor{blue}{C} indicates fixed/confirmed bug \\ 
\hline
\multirow{5}{*}{\shortstack[l]{\textbf{\textit{P1.} Fail in special}\\ \textbf{data type}}} & \multirow{5}{*}{\shortstack[l]{\textit{Object should not be created only to getClass} fails with Array,\\ while works with ArrayList;}} & \textit{PMD}: SingularField (327)  \\
 &  &  \textit{SonarQube}: String function use should be optimized for single characters (8)  / \textcolor{blue}C\\
 &  & \textit{SonarQube}: Objects should not be created only to getClass (5)\\
 &  & \textit{PMD}: RedundantFieldInitializer (3) \\
 & & \textit{SpotBugs}: ICAST\_BAD\_SHIFT\_AMOUNT (3) \\
 \hline
\multirow{5}{*}{\shortstack[l]{\textbf{\textit{P2.} Fail in compound}\\ \textbf{expression}}} & \multirow{5}{*}{\shortstack[l]{\textit{QBA\_QUESTIONABLE\_BOOLEAN\_ASSIGNMENT} fails \\when compound expression is involved, e.g., \\
	\textit{if (scanning = b == false)};}
} & \textit{ErrorProne}: ToStringReturnsNull  (28)  \\
 & & \textit{SpotBugs}: QBA\_QUESTIONABLE\_BOOLEAN\_ ASSIGNMENT  (26)   \\
 & & \textit{SpotBugs}: SA\_LOCAL\_SELF\_ASSIGNMENT  (26) \\
 & &  \textit{SonarQube}: Variables should not be self-assigned (5)\\
  & &  \textit{SonarQube}: Fields should not be initialized to default values  (3)   \\
\hline
\multirow{4}{*}{\shortstack[l]{\textbf{\textit{P3.} Fail in implicit}\\ \textbf{operation}}} & \multirow{4}{*}{\shortstack[l]{\textit{IntLongMath (Expression of type int may overflow before} \\\textit{assigning to a long)} fails when used in comparison expression \\(i.e., implicit assign), e.g., 
\textit{if (score $>=$ level $\times$ level $\times$ 1000);} }} & \textit{ErrorProne}: IntLongMath (135)  / \textcolor{blue}C  \\
 & & \textit{SonarQube}: Static fields should not be updated in constructors (72)  / \textcolor{blue}C \\
  & & \textit{SpotBugs}: DMI\_INVOKING\_TOSTRING\_ON\_ ARRAY (53) \\
 & &  \textit{ErrorProne}: ArrayEquals (11)  \\
 \hline
\multirow{4}{*}{\shortstack[l]{\textbf{\textit{P4.} Fail in multiple}\\ \textbf{calling operations}}} & \multirow{4}{*}{\shortstack[l]{\textit{AvoidPrintStackTrace} fails when involving multiple \\calling operations, e.g.,
\textit{json.exception().printStackTrace();} }} & \textit{PMD}: UseCollectionIsEmpty (399) \\
 & & \textit{PMD}: AvoidPrintStackTrace (20)  / \textcolor{blue}C \\
 & & \textit{PMD}: ClassCastExceptionWithToArray (5) \\
 & & \textit{PMD}: DontCallThreadRun (5) \\
\hline
\multirow{3}{*}{\shortstack[l]{\textbf{\textit{P5.} Fail in separated}\\ \textbf{expressions}}} & \multirow{3}{*}{\shortstack[l]{\textit{UseProperClassLoader} fails when \textit{getClassLoader} is used \\in separated expressions, e.g., 
\textit{Foo foo = new Foo();}  \\
\textit{ClassLoader classLoader = foo.getClassLoader();}}} & \textit{PMD}: UseProperClassLoader (68)  / \textcolor{blue}C  \\
& & \textit{ErrorProne}: ToStringReturnsNull (28)  / \textcolor{blue}C \\
& & \textit{PMD}: InstantiationToGetClass (19)  \\
& & \\
\hline
\multirow{4}{*}{\shortstack[l]{\textbf{\textit{P6.} Fail in}\\ \textbf{unnecessary brackets}}} & \multirow{4}{*}{\shortstack[l]{\textit{SimplifyConditional} fails with \textit{if(rhs != null \&\& (rhs instanceof} \\\textit{ CodeLocation))}, yet works when deleting the unnecessary \\ brackets on the second condition;}}   &  \textit{PMD}: ReturnEmptyArrayRatherThanNull (770) \\
 & & \textit{PMD}: SimplifyConditional (109) \\
 & & \textit{SonarQube}: Switch statements should not contain non-case labels (39)  \\
 \hline
\multirow{3}{*}{\shortstack[l]{\textbf{\textit{P7.} Fail in}\\ \textbf{variables}}} & \multirow{3}{*}{\shortstack[l]{\textit{FinalFieldCouldBeStatic} fails when assigning to an expression, \\e.g., \textit{private final double HALF\_PI = Math.PI $*$ 0.5}, \\yet works when assigning to a constant;}} & \textit{PMD}:	FinalFieldCouldBeStatic (209) \\
 & & \textit{PMD}: AvoidDecimalLiteralsInBigDecimalConstructor (20)\\
  & & \\
 \hline
\multirow{2}{*}{\textbf{Others}} & \multirow{2}{*}{\shortstack[l]{N/A}}  & \textit{PMD}: AvoidThrowingNullPointerException (772) \\
 & & \textit{PMD}: SimplifyBooleanExpressions (623) / \textcolor{blue}C  \\
 & & \textit{PMD}: StringToString (215) \\

%  & &  \textit{SonarQube}: Catches should be combined (96) \\
%  & & \textit{PMD}: ClassWithOnlyPrivateConstructorsShouldBeFinal (360) \\
%  & & \textit{PMD}: AvoidCatchingThrowable (11) \\
%  & & \textit{PMD}: UnnecessaryCaseChange (89) \\
%   & & \textit{SpotBugs}: HE\_EQUALS\_USE\_HASHCODE (3) \\
\hline
\end{tabular}
\label{tab:bug_rule_implement}
\end{table*}

% \textit{1) AvoidThrowingNullPointerException} fails with the throw \\ \textit{NullPointerException} used in method definition, e.g., \\\textit{public foo() throw NullPointerException}; \\
% 2) \textit{StringToString} fails with StringMethod().toString(), while \\works with String.toString();
